Dual Generator Offline Reinforcement Learning

In offline RL, constraining the learned policy to remain close to the data is essential to prevent the policy from outputting out-of-distribution (OOD) actions with erroneously overestimated values. In principle, generative adversarial networks (GAN) can provide an elegant solution to do so, with the discriminator directly providing a probability that quantifies distributional shift. However, in practice, GAN-based offline RL methods have not performed as well as alternative approaches, perhaps because the generator is trained to both fool the discriminator and maximize return -- two objectives that can be at odds with each other. In this paper, we show that the issue of conflicting objectives can be resolved by training two generators: one that maximizes return, with the other capturing the ``remainder'' of the data distribution in the offline dataset, such that the mixture of the two is close to the behavior policy. We show that not only does having two generators enable an effective GAN-based offline RL method, but also approximates a support constraint, where the policy does not need to match the entire data distribution, but only the slice of the data that leads to high long term performance. We name our method DASCO, for Dual-Generator Adversarial Support Constrained Offline RL. On benchmark tasks that require learning from sub-optimal data, DASCO significantly outperforms prior methods that enforce distribution constraint.

==> proof42_no_explicit_constraint.tex <==
We recall the theorem:

\thmjointinsupportmax*

\textit{Proof.} Similar to the proof for Theorem \ref{thm_disjoint}, we can rewrite the objective function in Eq.~\ref{eq:joint_gan} as:

\begin{align}
     & V(G, D^*_G)\\
     & = 2JSD( p_{\text{data}} || \dfrac{ p_g + p_{aux} }{ 2 } ) + \mathbb{E}_{x \sim p_g} [ f ( x ) ] - \log 4 
\end{align}

We then introduce the following notation changes: 
\begin{itemize}
    \item Let $g^{(i)} = p_g(x_i)$ be the probability that $p_g$ assigns to $x_i$  and $g = [g^{(1)}, \ldots, g^{(n)}]^T$. 
    \item Let $a^{(i)} = p_{aux}(x_i)$ be the probability that $p_{aux}$ assigns to $x_i$  and $a = [a^{(1)}, \ldots, a^{(n)}]^T$. 
    \item Let $f^{(i)} = f(x_i)$ be the value that the secondary objective $f$ assigns to $x_i$. Let $f = [f^{(1)}, \ldots, f^{(n)}]^T$. 
    \item Let $ p_{\text{data} }^{(i)} = p_{\text{data} } (x_i) $ be the probability that the data distribution assigns to $x_i$.
\end{itemize}

We can then rewrite the problem in Eq.~\ref{eq:joint_gan} in standard form \cite{boyd2004convex} as:
\begin{align}
\min_{g, a} \quad 2JSD( p_{\text{data}} & || \dfrac{ g + a }{ 2 } )  + g^T f \label{eq:proof_joint_gan_obj} \\
\textrm{s.t.} \quad - g^{(i)} &  \leq 0 \label{eq:proof_joint_gan_g_nonnegative}  \\
  \mathbf{1}^T g - 1 & = 0  \label{eq:proof_joint_gan_g_normalized} \\
 \quad - a^{(i)} & \leq 0 \label{eq:proof_joint_gan_aux_nonnegative}  \\
  \mathbf{1}^T a - 1 & = 0 \label{eq:proof_joint_gan_aux_normalized}
\end{align}

The optimization above is convex because the first time in the objective function is a composition of a convex function (the JSD) with an affine mapping ($ \dfrac{ g + a }{ 2 }$). Similarly to the proof for Theorem \ref{thm_disjoint}, strong duality holds.

The Lagrangian is:
\begin{align}
    L = 2JSD( p_{\text{data}} ||  \dfrac{ g + a }{ 2 } )  + g^T f - \sum_i {}^g\lambda^{(i)} g^{(i)} + {}^g\nu ( \mathbf{1}^T g - 1 ) - \sum_i {}^a\lambda^{(i)} a^{(i)} + {}^a\nu ( \mathbf{1}^T a - 1 )
\end{align}
where the association between the Lagrangian multipliers and constraints are as followed:
\begin{itemize}
    \item ${}^g\lambda^{(i)}$ is the multipliers for constraint \ref{eq:proof_joint_gan_g_nonnegative}
    \item ${}^g\nu$ is the multipliers for constraint \ref{eq:proof_joint_gan_g_normalized}
    \item ${}^a\lambda^{(i)}$ is the multipliers for constraint \ref{eq:proof_joint_gan_aux_nonnegative}
    \item ${}^a\nu$ is the multipliers for constraint \ref{eq:proof_joint_gan_aux_normalized}
\end{itemize}

Let $g_*$ and $({}^g\lambda^{(i)}_*, {}^g\nu_*, {}^a\lambda^{(i)}_*, {}^a\nu_*)$ be the primal and dual optimal solutions of the optimization problem. Because strong duality holds, the variables $g_*$ and $({}^g\lambda^{(i)}_*, {}^g\nu_*, {}^a\lambda^{(i)}_*, {}^a\nu_*)$ must satisfy the KKT conditions. For any $i \in [1, n]$, the following holds:
\begin{align}
    -g_*^{(i)} & \leq 0 \label{eq:proof_joint_gan_g_kkt_nonnegative} \\ 
    \mathbf{1}^T g_* - 1 & = 0 \\ 
   {}^g\lambda_*^{(i)} & \geq 0 \\ 
    {}^g\lambda_*^{(i)} g_*^{(i)} & = 0 \label{eq:proof_joint_gan_g_slack} \\ 
    \pdv{L}{ g^{(i)} } & = 0 \label{eq:proof_joint_gan_g_kkt_lang} \\
    -a_*^{(i)} & \leq 0 \label{eq:proof_joint_gan_a_kkt_nonnegative}  \\ 
    \mathbf{1}^T a_* - 1 & = 0 \\ 
   {}^a\lambda_*^{(i)} & \geq 0 \\ 
    {}^a\lambda_*^{(i)} a_*^{(i)} & = 0 \label{eq:proof_joint_gan_a_slack} \\ 
    \pdv{L}{ a^{(i)} } & = 0 \label{eq:proof_joint_gan_a_lang}
\end{align}
where the conditions \ref{eq:proof_joint_gan_g_kkt_nonnegative} to \ref{eq:proof_joint_gan_g_kkt_lang} are the KKT conditions associated with the decision variables $g$, and the conditions \ref{eq:proof_joint_gan_a_kkt_nonnegative} to \ref{eq:proof_joint_gan_a_lang} are the KKT conditions associated with the decision variables $a$.

We can show that the partial derivatives of the Lagrangian with respect to the variables $g, a$ are:

\begin{align}
    \pdv{L}{ g^{(i)} } & = f^{ (i) } - {}^g\lambda_*^{(i)} + {}^g\nu_* + \dfrac{1}{2} \log \left( \dfrac{ 2( a_*^{(i)} + g_*^{(i)} ) }{ a_*^{(i)} + 2p_{\text{data} }^{(i)} + g_*^{(i)} } \right) = 0 \label{eq:proof_joint_gan_pdvL_pdg} \\
    \pdv{L}{ a^{(i)} } & = - {}^a\lambda_*^{(i)} + {}^a\nu_* + \dfrac{1}{2} \log \left( \dfrac{ 2( a_*^{(i)} + g_*^{(i)} ) }{ a_*^{(i)} + 2p_{\text{data} }^{(i)} + g_*^{(i)} } \right) = 0 \label{eq:proof_joint_gan_pdvL_pda}
\end{align}

Substituting the values of ${}^g\lambda_*^{(i)}$ in \ref{eq:proof_joint_gan_pdvL_pdg} into \ref{eq:proof_joint_gan_g_slack} and ${}^a\lambda_*^{(i)}$ in \ref{eq:proof_joint_gan_pdvL_pda} into \ref{eq:proof_joint_gan_a_slack}, we have:

\begin{align}
    \left[ f^{ (i) } + {}^g\nu_* + \dfrac{1}{2} \log \left( \dfrac{ 2( a_*^{(i)} + g_*^{(i)} ) }{ a_*^{(i)} + 2p_{\text{data} }^{(i)} + g_*^{(i)} } \right) \right] g_*^{(i)} = 0 \label{eq:proof_joint_gan_comp_g} \\
    \left[ {}^a\nu_* + \dfrac{1}{2} \log \left( \dfrac{ 2( a_*^{(i)} + g_*^{(i)} ) }{ a_*^{(i)} + 2p_{\text{data} }^{(i)} + g_*^{(i)} } \right) \right] a_*^{(i)} = 0 \label{eq:proof_joint_gan_comp_a}
\end{align}

For each $i$, there are three cases we consider:
\begin{enumerate}
    \item $ g_*^{(i)} = 0, a_*^{(i)} > 0 $
    \item $ g_*^{(i)} > 0, a_*^{(i)} > 0 $
    \item $ g_*^{(i)} > 0, a_*^{(i)} = 0 $
\end{enumerate}
For example, in case $1.$, the primary generator assigns zero probability to $x_i$, but the auxiliary generator assigns non-zero probability to $x_i$.

Due to complementary slackness, we have the following results.

For case $1.$, we have from Eq.~\ref{eq:proof_joint_gan_comp_a} that:
\begin{align}
    g_*^{(i)} = 0, a_*^{(i)} > 0 & \Longrightarrow {}^a\nu_* + \dfrac{1}{2} \log \left( \dfrac{ 2( a_*^{(i)} + g_*^{(i)} ) }{ a_*^{(i)} + 2p_{\text{data} }^{(i)} + g_*^{(i)} } \right) = 0 \\ 
    & \Longrightarrow a_*^{(i)} = 2p_{\text{data} }^{(i)} \dfrac{ \exp{ [- 2{}^a\nu_*] } }{ 2 - \exp{ [- 2{}^a\nu_*] } }
\end{align}

For case $3.$, we have from Eq.~\ref{eq:proof_joint_gan_comp_g} that:
\begin{align}
    g_*^{(i)} > 0, a_*^{(i)} = 0 & \Longrightarrow f^{ (i) } + {}^g\nu_* + \dfrac{1}{2} \log \left( \dfrac{ 2( a_*^{(i)} + g_*^{(i)} ) }{ a_*^{(i)} + 2p_{\text{data} }^{(i)} + g_*^{(i)} } \right) = 0 \\
    & \Longrightarrow g_*^{(i)} = 2p_{\text{data} }^{(i)} \dfrac{ \exp{ [- 2f^{ (i) } - 2{}^g\nu_*] } }{ 2 - \exp{ [- 2f^{ (i) } - 2{}^g\nu_*] } }
\end{align}

For case $2.$, we have from Eq.~\ref{eq:proof_joint_gan_pdvL_pda} that:
\begin{align}
    g_*^{(i)} > 0, a_*^{(i)} > 0 \Longrightarrow g_*^{(i)} + a_*^{(i)} = 2p_{\text{data} }^{(i)} \dfrac{ \exp{ [- 2{}^a\nu_*] } }{ 2 - \exp{ [- 2{}^a\nu_*] } }
\end{align}

Since the primal problem \ref{eq:proof_joint_gan_obj}-\ref{eq:proof_joint_gan_aux_normalized} is convex, satisfying the KKT conditions are sufficient for any particular values of the decision variables $g, a$ and the Lagrange multipliers to be primal and dual optimal.

% We next restate the solutions for the decision variables $g, a$ that were stated in Section \ref{sec:dual_gen} and show that we can pick the values for the Lagrange multipliers such that the stated solutions for $g, a$ and the Lagrange multipliers satisfy the KKT conditions. Therefore, the stated solutions for $g, a$ are the optimal solution to the optimization problem \ref{eq:proof_joint_gan_obj}-\ref{eq:proof_joint_gan_aux_normalized}.

% The stated solutions for $g, a$ are as follows. We define $x_0$ to be the element inside the support of the data distribution $p_{\mathcal{D}}$ that minimizes $f$. Then:
% \begin{align}
%     p^*_{g} (x_0) & = \begin{cases}
%     2p_{\mathcal{D}} (x_0) \quad  \text{if} \quad 2p_{\mathcal{D}} (x_0) < 1 \\
%     1 \quad \quad  \quad \quad \text{otherwise}
%     \end{cases}
% \end{align}
% If the global maximum $x_0$ is not taking the full probability mass, the rest of the probability mass is redistributed to the next best in-support minima, which we can define recursively:
% \begin{align}
%          \text{For} \,\, x_i \in \underset{x \in \text{Supp}( p_{\mathcal{D}} ) \setminus \{ x_j \}_{j=0}^{i-1} }{\arg\min} f(x), \,\,
%     p^*_{g} (x_i) & = \begin{cases}
%       2p_{\mathcal{D}} (x_i)\quad \quad \quad \quad \quad \text{if} \quad \sum_{j=0}^i p^*_g(x_j) < 1 \\
%       1 -  \sum_{j=0}^{i-1} p^*_g(x_j) \quad \,\, \text{if} \quad \sum_{j=0}^i p^*_g(x_j) > 1 \\ 
%       0 \quad \quad \quad \quad \quad \quad \quad \quad  \text{if} \quad \sum_{j=0}^{i-1} p^*_g(x_j) = 1 
%     \end{cases}       
% \end{align}

% We set then the Lagrange multipliers as follows:
% \begin{align}
%     {}^a\nu_* & = 0 \\ 
%     {}^g\nu_* & = f(x_0)
% \end{align}

% We then have:
% \begin{align}
%     g_*^{(i)} = 0, a_*^{(i)} > 0 & \Longrightarrow a_*^{(i)} = 2p_{\text{data} }^{(i)} \\ 
%     g_*^{(i)} > 0, a_*^{(i)} > 0 & \Longrightarrow g_*^{(i)} + a_*^{(i)} = 2p_{\text{data} }^{(i)} \\ 
%     g_*^{(i)} > 0, a_*^{(i)} = 0 & \Longrightarrow g_*^{(i)} = 2p_{\text{data} }^{(i)}
% \end{align}
